UnSplit: Data-Oblivious Model Inversion, Model Stealing, and Label Inference Attacks Against Split Learning

Training deep neural networks often forces users to work in a distributed or outsourced setting, accompanied with privacy concerns. Split learning aims to address this concern by distributing the model among a client and a server. The scheme supposedly provides privacy, since the server cannot see the clients' models and inputs. We show that this is not true via two novel attacks. (1) We show that an honest-but-curious split learning server, equipped only with the knowledge of the client neural network architecture, can recover the input samples and obtain a functionally similar model to the client model, without being detected. (2) We show that if the client keeps hidden only the output layer of the model to "protect" the private labels, the honest-but-curious server can infer the labels with perfect accuracy. We test our attacks using various benchmark datasets and against proposed privacy-enhancing extensions to split learning. Our results show that plaintext split learning can pose serious risks, ranging from data (input) privacy to intellectual property (model parameters), and provide no more than a false sense of security.

==> figures/attack_visual.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.48\textwidth]{diagrams/attack_diagram.png}
    \caption{An illustration of UnSplit. On receiving the intermediate activations $f_1(x)$ from the client, the server tries to minimize the loss function $L$ to find input $\tilde{x}$ and model $\tilde{f_1}$ that result in a similar output to the intermediate activations received from the client.}
    \label{fig:attack_diagram}
\end{figure}

==> figures/comparisons.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}{0.8\linewidth}
        \centering
        \includegraphics[width=\textwidth]{diagrams/wb_qf_compare.png}
        \caption{Comparison with the query-free and white-box attacks in \citep{he_model_2019}.}
        \label{fig:qf_wb_compare}
    \end{subfigure}
    
    \vspace{0.3cm}
    
    \begin{subfigure}{0.8\linewidth}
        \centering
        \includegraphics[width=\textwidth]{diagrams/fsha_compare.png}
        \caption{Comparison with FSHA.}
        \label{fig:fsha_compare}
    \end{subfigure}
    
    \caption{Comparison of UnSplit with the attacks described in \citep{he_model_2019} for white box and query-free scenario, and FSHA \citep{pasquini_unleashing_2021}. The figures displays the MSE values between the estimated inputs and the original values averaged over possible split layers. The vertical lines represent the upper and lower quartiles of the values, while the bars correspond to the means.}
    \label{fig:comparisons}
\end{figure}



==> figures/epochs_mse.tex <==
\begin{figure*}[t]
    \begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\textwidth]{diagrams/mnist_epochs.png}
        \caption{MNIST}
        \label{fig:mnist_epochs}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\textwidth]{diagrams/f_mnist_epochs.png}
        \caption{Fashion-MNIST}
        \label{fig:f_mnist_epochs}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\textwidth]{diagrams/cifar_epochs.png}
        \caption{CIFAR10}
        \label{fig:cifar_epochs}
    \end{subfigure}
    
    \caption{MSE values of the estimated inputs after each training epoch, averaged over possible split layers. It can be observed that the estimates become more accurate as the client model is trained.}
    \label{fig:epochs_mse}
\end{figure*}

==> figures/labels_train.tex <==
\begin{figure}[t]
    \hspace{1cm}
    \begin{subfigure}{0.4\textwidth}
        \includegraphics[width=\textwidth]{diagrams/mnist_label_train.png}
        \caption{MNIST}
        \label{fig:mnist_label_train}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}{0.4\textwidth}
        \includegraphics[width=\textwidth]{diagrams/f_mnist_label_train.png}
        \caption{Fashion-MNIST}
        \label{fig:f_mnist_label_train}
    \end{subfigure}
    
    \caption{Classification performance of the original model and the clone model on unseen data for MNIST and Fashion-MNIST datasets. It can be seen that since the attacker can predict the labels with perfect accuracy, and can train its clone model accordingly, the two models follow very similar curves.}
    \label{fig:labels_train}
\end{figure}

==> tables/image_comparison.tex <==
\begin{table}[t!]
    \tabcolsep=0.05cm
    \begin{tabular}{cc}
        \toprule
        \multicolumn{2}{c}{\textbf{MNIST}} \\ \midrule
        GT & \includegraphics[width=0.42\textwidth]{results/mnist/targets.png} \\ 
        WB   & \includegraphics[width=0.42\textwidth]{results/comparison/mnist_wb_pool1.png} \\ 
        \textbf{US} & \includegraphics[width=0.42\textwidth]{results/mnist/after_train/pool1.png} \\ 
        QF  & \includegraphics[width=0.42\textwidth]{results/comparison/mnist_qf_pool1.png} \\ 
        \bottomrule
    \end{tabular}
    
    \vspace{0.3cm}
    
    \tabcolsep=0.05cm
    \begin{tabular}{cc}
        \toprule
        \multicolumn{2}{c}{\textbf{Fashion-MNIST}} \\ \midrule
        GT & \includegraphics[width=0.42\textwidth]{results/f_mnist/targets.png} \\ 
        WB & \includegraphics[width=0.42\textwidth]{results/comparison/f_mnist_wb_pool1.png} \\ 
        \textbf{US} & \includegraphics[width=0.42\textwidth]{results/f_mnist/after_train/pool1.png} \\ 
        QF & \includegraphics[width=0.42\textwidth]{results/comparison/f_mnist_qf_pool1.png} \\
        \bottomrule
    \end{tabular}
    
    \vspace{0.3cm}
    
    \tabcolsep=0.05cm
    \begin{tabular}{cc}
        \toprule
        \multicolumn{2}{c}{\textbf{CIFAR10}} \\ \midrule
        GT & \includegraphics[width=0.42\textwidth]{results/cifar/targets.png} \\ 
        WB & \includegraphics[width=0.42\textwidth]{results/comparison/cifar_wb_conv12.png} \\ 
        \textbf{US} &\includegraphics[width=0.42\textwidth]{results/cifar/after_train/conv12.png} \\ 
        QF & \includegraphics[width=0.42\textwidth]{results/comparison/cifar_qf_conv12.png} \\
        \bottomrule
    \end{tabular}
    
    \caption{Comparison of estimated inputs obtained from the white-box and query-free scenarios in \citep{he_model_2019} and UnSplit for the same split depth of three for each of our benchmark datasets. \textbf{WB} refers to \cite{he_model_2019}'s hite-box attack, and \textbf{QF} refers to their query-free attack. \textbf{US} refers to \textbf{U}n\textbf{S}plit and \textbf{GT} refers to the ground truth images.}
    \label{tab:comp_img}
\end{table}

==> tables/main_results_brief.tex <==
\begin{table}[t!]
    \caption{Estimated inputs before and after the training phase for MNIST, F-MNIST, and CIFAR10 datasets, width client model depths of 3, 3, and 5 respectively. The first row of each dataset displays the original inputs.\\}
    \label{tab:main_results_brief}
    
    \centering
    \begin{tabular}{cc}
        \toprule
        Before Training & After Training \\ \midrule
        \includegraphics[width=0.47\textwidth]{results/mnist/targets.png} & \includegraphics[width=0.47\textwidth]{results/mnist/targets.png}
        \\
        \includegraphics[width=0.47\textwidth]{results/mnist/before_train/pool1.png} & \includegraphics[width=0.47\textwidth]{results/mnist/after_train/pool1.png}
        \\ \midrule
        \includegraphics[width=0.47\textwidth]{results/f_mnist/targets.png} & \includegraphics[width=0.47\textwidth]{results/f_mnist/targets.png}
        \\
        \includegraphics[width=0.47\textwidth]{results/f_mnist/before_train/pool1.png} & \includegraphics[width=0.47\textwidth]{results/f_mnist/after_train/pool1.png}
        \\ \midrule
        \includegraphics[width=0.47\textwidth]{results/cifar/targets.png} & \includegraphics[width=0.47\textwidth]{results/cifar/targets.png}
        \\
        \includegraphics[width=0.47\textwidth]{results/cifar/before_train/pool1.png} & \includegraphics[width=0.47\textwidth]{results/cifar/after_train/pool1.png} 
        \\ \bottomrule
    \end{tabular}

\end{table}
